Skein theory for the ADE planar algebras

We give generators and relations for the planar algebras corresponding to $ADE$ subfactors. We also give a basis and an algorithm to express an arbitrary diagram as a linear combination of these basis diagrams.

==> makepdfs <==
#!/bin/sh

mpost manfig
for i in manfig.[1234567890]*
do
  n=`echo $i | sed 's/\.//'`.eps
  mv $i $n
  epstopdf $n
done

